A Survey of Few-Shot Learning on Graphs: from Meta-Learning to Pre-Training and Prompt Learning

Graph representation learning, a critical step in graph-centric tasks, has seen significant advancements. Earlier techniques often operate in an end-to-end setting, which heavily rely on the availability of ample labeled data. This constraint has spurred the emergence of few-shot learning on graphs, where only a few labels are available for each task. Given the extensive literature in this field, this survey endeavors to synthesize recent developments, provide comparative insights, and identify future directions. We systematically categorize existing studies based on two major taxonomies: (1) Problem taxonomy, which explores different types of data scarcity problems and their applications, and (2) Technique taxonomy, which details key strategies for addressing these data-scarce few-shot problems. The techniques can be broadly categorized into meta-learning, pre-training, and hybrid approaches, with a finer-grained classification in each category to aid readers in their method selection process. Within each category, we analyze the relationships among these methods and compare their strengths and limitations. Finally, we outline prospective directions for few-shot learning on graphs to catalyze continued innovation in this field. The website for this survey can be accessed by \url{https://github.com/smufang/fewshotgraph}.

==> sec-overview.tex <==
\section{Overview of Taxonomies}\label{sec.overview}
We categorizes the literature based on the perspectives of both problems and techniques, aiming to furnish a comprehensive overview.

% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{figures/Overview of Survey.png} 
% \caption{Overview framework of this survey.}
% \label{fig.overview}
% \end{figure}

\subsection{Taxonomy of Problems}
Regarding the taxonomy of problems, our analysis commences with an investigation into the research tasks associated with FSLG. Scarcity of data in graphs is multifaceted, a characteristic stemming from the inherent complexity of graph data. Specifically, this scarcity can be categorized into two types: label scarce and structural scarce. On one hand, the availability of labeled data may be limited in downstream tasks, leading to restricted supervisory information \cite{yu2023generalized,yu2023hgprompt}. On the other hand, the distinctiveness of graph structures can introduce another dimension of data scarce in graph learning models. For instance, the varying abundance of node neighborhoods \cite{liu2021tail,zheng2021cold} may lead to discrepancies in the information presented, potentially skewing the output of the learning model.

Consequently, we initially categorize FSLG based on the type of data scarcity, namely, label scarcity and structural scarcity. Given the distinct graph structures, we further subdivide the data scarcity into more nuanced categories based on graph-related elements, \textit{i.e.}, node-, edge-, and graph-level elements, thereby gaining a more detailed perspective on these issues. Figure~\ref{fig.intro-framework} illustrates this taxonomy of problems.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/Taxonomy of problem.png} 
\caption{Taxonomy of problems.}
\label{fig.taxonomy-problem}
\end{figure}

\subsection{Taxonomy of Techniques}
In the taxonomy of techniques, the survey is categorized based on strategies employed to mitigate the few-shot issue, as summarized in Figure~\ref{fig.intro-framework}. Initially, techniques are separated based on whether they leverage meta-knowledge or pre-trained knowledge, resulting in two primary categories: meta-learning on graphs and pre-training on graphs. In meta-learning on graphs, based on the enhancement strategy, further categorization includes structure- and adaptation-based enhancements, among others. In pre-training on graphs, further categorization is based on pre-training strategies, namely, contrastive learning, generative methods, and hybrid methods; as well as various tuning strategies, including classical fine-tuning, parameter-efficient fine-tuning, and prompting. Subsequently, the major techniques employed to address imbalance issues in each branch are summarized, with detailed illustrations provided for techniques under each main category.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/Taxonomy of technique.png} 
\caption{Taxonomy of techniques.}
\label{fig.taxonomy-technique}
\end{figure}

\stitle{Organization.}
In the subsequent three sections, this survey introduces the two taxonomies of FSLG. Specifically, Sections~\ref{sec.pro} address the problems of FSLG, focusing on data scarce and structural scarce, respectively. In Sections~\ref{sec.meta-learning} and~\ref{sec.pre-training}, the survey classifies the relevant literature based on techniques for addressing few-shot issues, offering guidance to assist readers in selecting appropriate solutions. Section~\ref{sec.future} explores future research directions from both problem and technique perspectives, while Section~\ref{sec.conclusion} provides the survey's conclusion.
